Teaching Type Systems Implementation with Stella, an Extensible Statically Typed Programming Language

We report on a half-semester course focused around implementation of type systems in programming languages. The course assumes basics of classical compiler construction, in particular, the abstract syntax representation, the Visitor pattern, and parsing. The course is built around a language Stella with a minimalistic core and a set of small extensions, covering algebraic data types, references, exceptions, exhaustive pattern matching, subtyping, recursive types, universal polymorphism, and type reconstruction. Optionally, an implementation of an interpreter and a compiler is offered to the students. To facilitate fast development and variety of implementation languages we rely on the BNF Converter tool and provide templates for the students in multiple languages. Finally, we report some results of teaching based on students' achievements.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Stephen Chang (Ed.): Trends in Functional\\ Programming in Education (TFPIE)
\\
EPTCS 405, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.405.1}{10.4204/EPTCS.405.1}}

